Language Models as Inductive Reasoners

Inductive reasoning is a core component of human intelligence. In the past research of inductive reasoning within computer science, formal language is used as representations of knowledge (facts and rules, more specifically). However, formal language can cause systematic problems for inductive reasoning such as disability of handling raw input such as natural language, sensitiveness to mislabeled data, and incapacity to handle ambiguous input. To this end, we propose a new paradigm (task) for inductive reasoning, which is to induce natural language rules from natural language facts, and create a dataset termed DEER containing 1.2k rule-fact pairs for the task, where rules and facts are written in natural language. New automatic metrics are also proposed and analysed for the evaluation of this task. With DEER, we investigate a modern approach for inductive reasoning where we use natural language as representation for knowledge instead of formal language and use pretrained language models as ''reasoners''. Moreover, we provide the first and comprehensive analysis of how well pretrained language models can induce natural language rules from natural language facts. We also propose a new framework drawing insights from philosophy literature for this task, which we show in the experiment section that surpasses baselines in both automatic and human evaluations. We discuss about our future perspectives for inductive reasoning in Section 7. Dataset and code are available at https://github.com/ZonglinY/Inductive_Reasoning.

==> figures/recall_rate_figure.tex <==
\begin{figure}[t]
\centering
\resizebox{0.8\columnwidth}{!}{
\includegraphics[]{figures/Recall_rate.png}
}
\caption{Illustration of WRecall, one of our proposed automatic evaluation metric. Here weight reflects the importance level of each block of generated rules.}
\label{fig:recall_rate}
\end{figure}

==> tables/appen_analysis_rule_templates_finetuning.tex <==
\begin{table}[]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|cccc}
\toprule
Models & \thead{If \_\_,\\ then \_\_.} & \thead{There exists \_\_,\\ which \_\_.} & \thead{If \_\_ and \_\_,\\ then \_\_.} & \thead{If \_\_ or \_\_,\\ then \_\_.} \\ \midrule
R+F    & 9.87 / 2.22       & 17.45 / 2.95       & 10.63 / 2.30     & 12.53 / 2.50    \\
M1     & 22.65 / 3.37      & 31.92 / 4.00       & 26.25 / 3.62     & 28.75 / 3.79    \\ \midrule
M1+M2  & 25.23 / 3.90      & 34.32 / 4.52       & \textbf{27.37} / \textbf{3.90}     & 28.83 / 3.81    \\
M1+M3  & 26.01 / \textbf{4.11}      & 32.29 / 4.06       & 25.74 / 3.51     & 28.96 / 3.86    \\
M1+M4  & 24.80 / 3.96      & 33.58 / 4.47       & 25.61 / 3.50     & 29.83 / \textbf{4.11}    \\
M1+M5  & 23.16 / 3.55      & 32.79 / 4.26       & 26.40 / 3.65     & 29.18 / 3.92    \\
CoLM   & \textbf{27.03} / 3.97      & \textbf{36.27} / \textbf{4.84}       & 26.23 / 3.61     & \textbf{29.92} / 3.96    \\ \bottomrule
\end{tabular}}
\caption{Analysis of PLM~(GPT-J)'s performance (measured in METEOR / GREEN) in with different rule templates~(Under finetuning setting).}
\label{appen:analysis:rule_templates_finetune}
\end{table}

==> tables/appen_analysis_specific_general_facts.tex <==
\begin{table}[]
\centering
\resizebox{0.65\columnwidth}{!}{
\begin{tabular}{c|cc}
\toprule
Models & Specific facts & General facts \\ \midrule
R+F    & 10.15  / 2.25  & 12.79 / 2.53  \\
M1     & 26.37 / 3.63   & 24.18 / 3.48  \\ \midrule
M1+M2  & 27.57  / 3.91  & 27.90 / \textbf{4.23}  \\
M1+M3  & 27.43 / 3.92   & 27.44 / 4.17  \\
M1+M4  & 27.33 / 3.95   & 26.17 / 3.98  \\
M1+M5  & 26.74 / 3.73   & 24.84 / 3.70  \\
CoLM   & \textbf{28.62} / \textbf{3.98}   & \textbf{29.81} / 4.22  \\ \bottomrule
\end{tabular}}

\caption{Analysis of PLM~(GPT-J)'s performance (measured in METEOR / GREEN) in with specific or general input facts~(Under finetuning setting).}
\label{appen:analysis_specific_general_finetune}
\end{table}

==> tables/appen_analysis_topics_finetuning.tex <==
\begin{table}[]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|cccccc}
\toprule
\multicolumn{1}{c}{Models} & Zoology      & Botany       & Astronomy    & Geology      & History      & Physics      \\ \midrule
R+F                        & 9.65 / 2.20  & 10.24 / 2.26 & 13.09 / 2.56 & 13.28 / 2.58 & 11.07 / 2.35 & 11.44 / 2.39 \\
M1                         & 29.29 / 3.83 & 30.47 / 3.90 & 34.01 / 4.12 & 28.28 / 3.83 & 23.61 / 3.44 & 18.69 / 3.06 \\ \midrule
M1+M2                      & \textbf{29.46} / \textbf{3.90} & 30.44 / 3.90 & 38.30 / 4.88 & 29.31 / 4.03 & 25.18 / \textbf{3.78} & 22.46 / 3.75 \\
M1+M3                      & 28.67 / 3.65 & 30.28 / 3.88 & 42.63 / 5.13 & 30.04 / \textbf{4.29} & 24.55 / 3.66 & 22.36 / 3.66 \\
M1+M4                      & 26.75 / 3.18 & 31.90 / \textbf{4.35} & 34.97 / 4.43 & 29.27 / 4.11 & 24.12 / 3.57 & 21.20 / 3.66 \\
M1+M5                      & 29.34 / 3.80 & 31.14 / 4.13 & 34.57 / 4.28 & 29.15 / 4.06 & 23.60 / 3.41 & 19.34 / 3.28 \\
CoLM                       & 28.85 / 3.68 & \textbf{32.97} / 4.29 & \textbf{45.70} / \textbf{5.25} & \textbf{30.38} / 4.18 & \textbf{25.36} / 3.70 & \textbf{27.72} / \textbf{4.01} \\ \bottomrule
\end{tabular}}
\caption{Analysis of PLM~(GPT-J)'s performance~(measured in METEOR / GREEN) in under different topics~(Under finetuning setting).}
\label{appen:analysis:topics_finetune}
\end{table}
